Tweet Sentiment Quantification: An Experimental Re-Evaluation

Sentiment quantification is the task of training, by means of supervised learning, estimators of the relative frequency (also called ``prevalence'') of sentiment-related classes (such as \textsf{Positive}, \textsf{Neutral}, \textsf{Negative}) in a sample of unlabelled texts. This task is especially important when these texts are tweets, since the final goal of most sentiment classification efforts carried out on Twitter data is actually quantification (and not the classification of individual tweets). It is well-known that solving quantification by means of ``classify and count'' (i.e., by classifying all unlabelled items by means of a standard classifier and counting the items that have been assigned to a given class) is less than optimal in terms of accuracy, and that more accurate quantification methods exist. Gao and Sebastiani (2016) carried out a systematic comparison of quantification methods on the task of tweet sentiment quantification. In hindsight, we observe that the experimental protocol followed in that work was weak, and that the reliability of the conclusions that were drawn from the results is thus questionable. We now re-evaluate those quantification methods (plus a few more modern ones) on exactly the same same datasets, this time following a now consolidated and much more robust experimental protocol (which also involves simulating the presence, in the test data, of class prevalence values very different from those of the training set). This experimental protocol (even without counting the newly added methods) involves a number of experiments 5,775 times larger than that of the original study. The results of our experiments are dramatically different from those obtained by Gao and Sebastiani, and they provide a different, much more solid understanding of the relative strengths and weaknesses of different sentiment quantification methods.

==> tab_rank_mae.tex <==
\begin{tabularx}{\textwidth}{|c||Y|Y|Y|Y|Y|Y|Y|Y|} \hline
          & \multicolumn{8}{c|}{Methods tested in~\cite{Gao:2016uq}}  \\ \hline
     & \side{CC$^{\mathrm{AE}}$}  & \side{ACC$^{\mathrm{AE}}$}  & \side{PCC$^{\mathrm{AE}}$}  & \side{PACC$^{\mathrm{AE}}$}  & \side{EMQ$^{\mathrm{AE}}$}  & \side{SVM(Q)$^{\mathrm{AE}}$}  & \side{SVM(KLD)$^{\mathrm{AE}}$}  & \side{SVM(NKLD)$^{\mathrm{AE}}$} \\\hline
GASP  & 4\cellcolor{green!7} (5) & 2\cellcolor{green!35} (3) & 8\cellcolor{red!50} (2) & 3\cellcolor{green!21} (1) & 1\cellcolor{green!50} (6) & 7\cellcolor{red!35} (8) & 6\cellcolor{red!21} (4) & 5\cellcolor{red!7} (7)\\\hline
HCR  & 4\cellcolor{green!7} (5) & 3\cellcolor{green!21} (2) & 8\cellcolor{red!50} (1) & 2\cellcolor{green!35} (3) & 1\cellcolor{green!50} (7) & 7\cellcolor{red!35} (8) & 6\cellcolor{red!21} (4) & 5\cellcolor{red!7} (6)\\\hline
OMD  & 4\cellcolor{green!7} (6) & 2\cellcolor{green!35} (3) & 6\cellcolor{red!21} (1) & 3\cellcolor{green!21} (2) & 1\cellcolor{green!50} (8) & 8\cellcolor{red!50} (7) & 5\cellcolor{red!7} (4) & 7\cellcolor{red!35} (5)\\\hline
Sanders  & 5\cellcolor{red!7} (5) & 2\cellcolor{green!35} (4) & 8\cellcolor{red!50} (2) & 3\cellcolor{green!21} (3) & 1\cellcolor{green!50} (6) & 6\cellcolor{red!21} (8) & 7\cellcolor{red!35} (1) & 4\cellcolor{green!7} (7)\\\hline
SemEval13  & 4\cellcolor{green!7} (7) & 2\cellcolor{green!35} (5) & 8\cellcolor{red!50} (1) & 1\cellcolor{green!50} (6) & 3\cellcolor{green!21} (8) & 5\cellcolor{red!7} (4) & 7\cellcolor{red!35} (3) & 6\cellcolor{red!21} (2)\\\hline
SemEval14  & 4\cellcolor{green!7} (8) & 2\cellcolor{green!35} (2) & 8\cellcolor{red!50} (6) & 1\cellcolor{green!50} (1) & 3\cellcolor{green!21} (3) & 6\cellcolor{red!21} (7) & 7\cellcolor{red!35} (5) & 5\cellcolor{red!7} (4)\\\hline
SemEval15  & 4\cellcolor{green!7} (4) & 2\cellcolor{green!35} (3) & 8\cellcolor{red!50} (1) & 3\cellcolor{green!21} (2) & 1\cellcolor{green!50} (7) & 5\cellcolor{red!7} (8) & 7\cellcolor{red!35} (6) & 6\cellcolor{red!21} (5)\\\hline
SemEval16  & 3\cellcolor{green!21} (3) & 5\cellcolor{red!7} (4) & 8\cellcolor{red!50} (1) & 2\cellcolor{green!35} (7) & 1\cellcolor{green!50} (5) & 7\cellcolor{red!35} (8) & 4\cellcolor{green!7} (2) & 6\cellcolor{red!21} (6)\\\hline
SST  & 5\cellcolor{red!7} (2) & 3\cellcolor{green!21} (5) & 8\cellcolor{red!50} (1) & 2\cellcolor{green!35} (8) & 1\cellcolor{green!50} (3) & 7\cellcolor{red!35} (6) & 4\cellcolor{green!7} (4) & 6\cellcolor{red!21} (7)\\\hline
WA  & 5\cellcolor{red!7} (6) & 3\cellcolor{green!21} (5) & 6\cellcolor{red!21} (2) & 1\cellcolor{green!50} (1) & 2\cellcolor{green!35} (3) & 8\cellcolor{red!50} (8) & 7\cellcolor{red!35} (7) & 4\cellcolor{green!7} (4)\\\hline
WB  & 4\cellcolor{green!7} (2) & 3\cellcolor{green!21} (4) & 5\cellcolor{red!7} (1) & 2\cellcolor{green!35} (3) & 1\cellcolor{green!50} (5) & 8\cellcolor{red!50} (6) & 6\cellcolor{red!21} (8) & 7\cellcolor{red!35} (7)\\\hline
\end{tabularx}
       

==> tab_rank_mrae.tex <==
\begin{tabularx}{\textwidth}{|c||Y|Y|Y|Y|Y|Y|Y|Y|} \hline
          & \multicolumn{8}{c|}{Methods tested in~\cite{Gao:2016uq}}  \\ \hline
     & \side{CC$^{\mathrm{RAE}}$}  & \side{ACC$^{\mathrm{RAE}}$}  & \side{PCC$^{\mathrm{RAE}}$}  & \side{PACC$^{\mathrm{RAE}}$}  & \side{EMQ$^{\mathrm{RAE}}$}  & \side{SVM(Q)$^{\mathrm{RAE}}$}  & \side{SVM(KLD)$^{\mathrm{RAE}}$}  & \side{SVM(NKLD)$^{\mathrm{RAE}}$} \\\hline
GASP  & 4\cellcolor{green!7} (5) & 3\cellcolor{green!21} (4) & 7\cellcolor{red!35} (3) & 2\cellcolor{green!35} (2) & 1\cellcolor{green!50} (6) & 8\cellcolor{red!50} (8) & 5\cellcolor{red!7} (1) & 6\cellcolor{red!21} (7)\\\hline
HCR  & 4\cellcolor{green!7} (4) & 2\cellcolor{green!35} (2) & 7\cellcolor{red!35} (1) & 3\cellcolor{green!21} (3) & 1\cellcolor{green!50} (7) & 8\cellcolor{red!50} (8) & 6\cellcolor{red!21} (5) & 5\cellcolor{red!7} (6)\\\hline
OMD  & 4\cellcolor{green!7} (6) & 2\cellcolor{green!35} (3) & 5\cellcolor{red!7} (1) & 3\cellcolor{green!21} (2) & 1\cellcolor{green!50} (8) & 8\cellcolor{red!50} (7) & 6\cellcolor{red!21} (4) & 7\cellcolor{red!35} (5)\\\hline
Sanders  & 4\cellcolor{green!7} (5) & 2\cellcolor{green!35} (4) & 7\cellcolor{red!35} (1) & 3\cellcolor{green!21} (3) & 1\cellcolor{green!50} (6) & 8\cellcolor{red!50} (8) & 6\cellcolor{red!21} (2) & 5\cellcolor{red!7} (7)\\\hline
SemEval13  & 4\cellcolor{green!7} (7) & 3\cellcolor{green!21} (3) & 6\cellcolor{red!21} (1) & 2\cellcolor{green!35} (4) & 1\cellcolor{green!50} (8) & 8\cellcolor{red!50} (6) & 5\cellcolor{red!7} (2) & 7\cellcolor{red!35} (5)\\\hline
SemEval14  & 4\cellcolor{green!7} (4) & 2\cellcolor{green!35} (2) & 6\cellcolor{red!21} (8) & 3\cellcolor{green!21} (3) & 1\cellcolor{green!50} (6) & 8\cellcolor{red!50} (7) & 5\cellcolor{red!7} (1) & 7\cellcolor{red!35} (5)\\\hline
SemEval15  & 4\cellcolor{green!7} (3) & 2\cellcolor{green!35} (5) & 6\cellcolor{red!21} (1) & 3\cellcolor{green!21} (2) & 1\cellcolor{green!50} (4) & 8\cellcolor{red!50} (8) & 5\cellcolor{red!7} (6) & 7\cellcolor{red!35} (7)\\\hline
SemEval16  & 4\cellcolor{green!7} (3) & 3\cellcolor{green!21} (5) & 6\cellcolor{red!21} (2) & 2\cellcolor{green!35} (7) & 1\cellcolor{green!50} (4) & 8\cellcolor{red!50} (8) & 5\cellcolor{red!7} (1) & 7\cellcolor{red!35} (6)\\\hline
SST  & 6\cellcolor{red!21} (3) & 3\cellcolor{green!21} (5) & 7\cellcolor{red!35} (1) & 2\cellcolor{green!35} (6) & 1\cellcolor{green!50} (2) & 8\cellcolor{red!50} (7) & 5\cellcolor{red!7} (4) & 4\cellcolor{green!7} (8)\\\hline
WA  & 5\cellcolor{red!7} (5) & 2\cellcolor{green!35} (4) & 6\cellcolor{red!21} (2) & 3\cellcolor{green!21} (1) & 1\cellcolor{green!50} (3) & 8\cellcolor{red!50} (8) & 7\cellcolor{red!35} (7) & 4\cellcolor{green!7} (6)\\\hline
WB  & 5\cellcolor{red!7} (2) & 2\cellcolor{green!35} (4) & 7\cellcolor{red!35} (1) & 3\cellcolor{green!21} (3) & 1\cellcolor{green!50} (5) & 8\cellcolor{red!50} (6) & 6\cellcolor{red!21} (8) & 4\cellcolor{green!7} (7)\\\hline
\end{tabularx}


==> tab_results_ae_ae.tex <==

            \resizebox{\textwidth}{!}{%
                    \begin{tabular}{|c|c||c|c|c|c|c|c|c|c||c|c|c|c|c|} \hline
                      & & \multicolumn{8}{c||}{Methods tested in~\cite{Gao:2016uq}} & 
                        \multicolumn{5}{c|}{Newly added methods} \\ \hline
                     & & \side{CC$^{\mathrm{AE}}$} & \side{ACC$^{\mathrm{AE}}$} & \side{PCC$^{\mathrm{AE}}$} & \side{PACC$^{\mathrm{AE}}$} & \side{SLD$^{\mathrm{AE}}$} & \side{SVM(Q)$^{\mathrm{AE}}$} & \side{SVM(KLD)$^{\mathrm{AE}}$} & \side{SVM(NKLD)$^{\mathrm{AE}}$} & \side{SVM(AE)$^{\mathrm{AE}}$} & \side{E(PACC)$_\mathrm{Ptr}^{\mathrm{AE}}$} & \side{E(PACC)$_\mathrm{AE}^{\mathrm{AE}}$} & \side{HDy$^{\mathrm{AE}}$} & \side{QuaNet$^{\mathrm{AE}}$} \\\hline
\multirow{12}{*}{\side{AE}} & GASP &  0.093 \cellcolor{red!3} &  0.052 \cellcolor{green!40} &  0.124 \cellcolor{red!36} &  0.044$^{\phantom{\ddag}}$ \cellcolor{green!48} & \textbf{0.043} \cellcolor{green!50} &  0.119 \cellcolor{red!31} &  0.114 \cellcolor{red!26} &  0.110 \cellcolor{red!21} &  0.136 \cellcolor{red!50} &  0.065 \cellcolor{green!25} &  0.049$^{\phantom{\ddag}}$ \cellcolor{green!43} &  0.086 \cellcolor{green!3} &  0.046$^{\phantom{\ddag}}$ \cellcolor{green!46} \\\cline{2-15}
& HCR &  0.130 \cellcolor{red!18} &  0.102 \cellcolor{green!12} &  0.158 \cellcolor{red!50} &  0.074$^{\phantom{\ddag}}$ \cellcolor{green!45} &  0.078 \cellcolor{green!40} &  0.150 \cellcolor{red!40} &  0.143 \cellcolor{red!33} &  0.138 \cellcolor{red!27} &  0.158 \cellcolor{red!49} &  0.084 \cellcolor{green!33} &  0.071$^{\dag\phantom{\dag}}$ \cellcolor{green!48} & \textbf{0.070} \cellcolor{green!50} &  0.099$^{\phantom{\ddag}}$ \cellcolor{green!17} \\\cline{2-15}
& OMD &  0.114 \cellcolor{red!17} &  0.086 \cellcolor{green!14} &  0.126 \cellcolor{red!32} &  0.067$^{\phantom{\ddag}}$ \cellcolor{green!37} & \textbf{0.055} \cellcolor{green!50} &  0.141 \cellcolor{red!50} &  0.124 \cellcolor{red!30} &  0.139 \cellcolor{red!47} &  0.116 \cellcolor{red!20} &  0.084 \cellcolor{green!16} &  0.075$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.119 \cellcolor{red!24} &  0.087$^{\phantom{\ddag}}$ \cellcolor{green!12} \\\cline{2-15}
& Sanders &  0.114 \cellcolor{red!12} &  0.058 \cellcolor{green!38} &  0.138 \cellcolor{red!33} &  0.049$^{\phantom{\ddag}}$ \cellcolor{green!46} & \textbf{0.045} \cellcolor{green!50} &  0.140 \cellcolor{red!35} &  0.141 \cellcolor{red!35} &  0.110 \cellcolor{red!8} &  0.157 \cellcolor{red!50} &  0.076 \cellcolor{green!22} &  0.058$^{\phantom{\ddag}}$ \cellcolor{green!37} &  0.087 \cellcolor{green!12} &  0.079$^{\phantom{\ddag}}$ \cellcolor{green!19} \\\cline{2-15}
& SemEval13 &  0.115 \cellcolor{red!5} &  0.086 \cellcolor{green!37} &  0.143 \cellcolor{red!47} & \textbf{0.078}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.097 \cellcolor{green!20} &  0.129 \cellcolor{red!26} &  0.144 \cellcolor{red!50} &  0.134 \cellcolor{red!34} &  0.143 \cellcolor{red!49} &  0.102 \cellcolor{green!12} &  0.093$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.114 \cellcolor{red!4} &  0.078$^{\ddag}$ \cellcolor{green!49} \\\cline{2-15}
& SemEval14 &  0.105 \cellcolor{red!11} &  0.060 \cellcolor{green!43} &  0.136 \cellcolor{red!50} & \textbf{0.054}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.076 \cellcolor{green!23} &  0.127 \cellcolor{red!38} &  0.128 \cellcolor{red!40} &  0.122 \cellcolor{red!32} &  0.134 \cellcolor{red!47} &  0.096 \cellcolor{red!1} &  0.067$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.083 \cellcolor{green!15} &  0.059$^{\phantom{\ddag}}$ \cellcolor{green!44} \\\cline{2-15}
& SemEval15 &  0.128 \cellcolor{red!7} &  0.103 \cellcolor{green!40} &  0.148 \cellcolor{red!47} &  0.101$^{\dag\phantom{\dag}}$ \cellcolor{green!44} &  0.104 \cellcolor{green!39} &  0.143 \cellcolor{red!36} &  0.150 \cellcolor{red!50} &  0.145 \cellcolor{red!40} &  0.144 \cellcolor{red!39} &  0.114 \cellcolor{green!19} &  0.112$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.105 \cellcolor{green!37} & \textbf{0.098}$^{\phantom{\ddag}}$ \cellcolor{green!50} \\\cline{2-15}
& SemEval16 &  0.146 \cellcolor{red!8} &  0.147 \cellcolor{red!9} &  0.171 \cellcolor{red!40} &  0.118$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{0.102} \cellcolor{green!50} &  0.167 \cellcolor{red!35} &  0.154 \cellcolor{red!18} &  0.165 \cellcolor{red!32} &  0.178 \cellcolor{red!50} &  0.131 \cellcolor{green!11} &  0.132$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.167 \cellcolor{red!35} &  0.103$^{\ddag}$ \cellcolor{green!47} \\\cline{2-15}
& SST &  0.110 \cellcolor{red!15} &  0.083 \cellcolor{green!15} &  0.140 \cellcolor{red!50} &  0.057$^{\phantom{\ddag}}$ \cellcolor{green!45} & \textbf{0.054} \cellcolor{green!50} &  0.136 \cellcolor{red!46} &  0.113 \cellcolor{red!19} &  0.128 \cellcolor{red!36} &  0.126 \cellcolor{red!33} &  0.063 \cellcolor{green!38} &  0.054$^{\ddag}$ \cellcolor{green!49} &  0.097 \cellcolor{red!0} &  0.069$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-15}
& WA &  0.082 \cellcolor{red!10} &  0.056 \cellcolor{green!24} &  0.082 \cellcolor{red!10} &  0.043$^{\phantom{\ddag}}$ \cellcolor{green!41} & \textbf{0.037} \cellcolor{green!50} &  0.111 \cellcolor{red!50} &  0.100 \cellcolor{red!34} &  0.063 \cellcolor{green!14} &  0.071 \cellcolor{green!4} &  0.043 \cellcolor{green!42} &  0.041$^{\phantom{\ddag}}$ \cellcolor{green!44} &  0.043 \cellcolor{green!42} &  0.053$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-15}
& WB &  0.077 \cellcolor{red!11} &  0.043 \cellcolor{green!35} &  0.083 \cellcolor{red!19} &  0.035$^{\phantom{\ddag}}$ \cellcolor{green!46} & \textbf{0.032} \cellcolor{green!50} &  0.106 \cellcolor{red!50} &  0.084 \cellcolor{red!19} &  0.103 \cellcolor{red!46} &  0.069 \cellcolor{red!0} &  0.048 \cellcolor{green!28} &  0.041$^{\phantom{\ddag}}$ \cellcolor{green!37} &  0.044 \cellcolor{green!33} &  0.046$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-15}
\cline{2-15}
& Average &  0.110 \cellcolor{red!16} &  0.080$^{\ddag}$ \cellcolor{green!28} &  0.132 \cellcolor{red!47} & \textbf{0.065} \cellcolor{green!50} &  0.066$^{\ddag}$ \cellcolor{green!49} &  0.134 \cellcolor{red!50} &  0.127 \cellcolor{red!40} &  0.123 \cellcolor{red!35} &  0.130 \cellcolor{red!45} &  0.082$^{\ddag}$ \cellcolor{green!25} &  0.072$^{\ddag}$ \cellcolor{green!40} &  0.092$^{\dag\phantom{\dag}}$ \cellcolor{green!10} &  0.074$^{\ddag}$ \cellcolor{green!36} \\\hline


\multirow{12}{*}{\side{KLD}} & GASP &  0.082 \cellcolor{green!5} &  0.045 \cellcolor{green!34} &  0.127 \cellcolor{red!29} &  0.029 \cellcolor{green!46} & \textbf{0.025}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.119 \cellcolor{red!23} &  0.113 \cellcolor{red!18} &  0.106 \cellcolor{red!12} &  0.154 \cellcolor{red!50} &  0.049 \cellcolor{green!31} &  0.029 \cellcolor{green!46} &  0.079 \cellcolor{green!7} &  0.028 \cellcolor{green!47} \\\cline{2-15}
& HCR &  0.141 \cellcolor{red!15} &  0.176 \cellcolor{red!40} &  0.188 \cellcolor{red!50} &  0.094 \cellcolor{green!19} &  0.062$^{\phantom{\ddag}}$ \cellcolor{green!43} &  0.172 \cellcolor{red!37} &  0.164 \cellcolor{red!32} &  0.154 \cellcolor{red!24} &  0.184 \cellcolor{red!46} &  0.075 \cellcolor{green!33} & \textbf{0.053} \cellcolor{green!50} &  0.078 \cellcolor{green!31} &  0.091 \cellcolor{green!22} \\\cline{2-15}
& OMD &  0.112 \cellcolor{green!0} &  0.099 \cellcolor{green!9} &  0.136 \cellcolor{red!17} &  0.076 \cellcolor{green!26} & \textbf{0.043}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.156 \cellcolor{red!31} &  0.132 \cellcolor{red!13} &  0.152 \cellcolor{red!28} &  0.119 \cellcolor{red!4} &  0.071 \cellcolor{green!30} &  0.061 \cellcolor{green!37} &  0.182 \cellcolor{red!50} &  0.078 \cellcolor{green!24} \\\cline{2-15}
& Sanders &  0.114 \cellcolor{red!9} &  0.048 \cellcolor{green!34} &  0.151 \cellcolor{red!33} &  0.030 \cellcolor{green!46} & \textbf{0.025}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.154 \cellcolor{red!36} &  0.155 \cellcolor{red!36} &  0.105 \cellcolor{red!3} &  0.175 \cellcolor{red!50} &  0.058 \cellcolor{green!28} &  0.041 \cellcolor{green!39} &  0.105 \cellcolor{red!3} &  0.063 \cellcolor{green!24} \\\cline{2-15}
& SemEval13 &  0.110 \cellcolor{red!0} &  0.087 \cellcolor{green!23} &  0.159 \cellcolor{red!50} &  0.075 \cellcolor{green!34} &  0.082$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.134 \cellcolor{red!24} &  0.157 \cellcolor{red!47} &  0.142 \cellcolor{red!32} &  0.158 \cellcolor{red!48} &  0.097 \cellcolor{green!13} &  0.080 \cellcolor{green!30} &  0.148 \cellcolor{red!38} & \textbf{0.060} \cellcolor{green!50} \\\cline{2-15}
& SemEval14 &  0.097 \cellcolor{red!2} &  0.057 \cellcolor{green!36} &  0.148 \cellcolor{red!50} &  0.051 \cellcolor{green!41} &  0.060$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.131 \cellcolor{red!33} &  0.131 \cellcolor{red!33} &  0.123 \cellcolor{red!26} &  0.143 \cellcolor{red!45} &  0.089 \cellcolor{green!6} &  0.054 \cellcolor{green!38} &  0.093 \cellcolor{green!1} & \textbf{0.042} \cellcolor{green!50} \\\cline{2-15}
& SemEval15 &  0.135 \cellcolor{red!4} &  0.115 \cellcolor{green!20} &  0.166 \cellcolor{red!42} &  0.123 \cellcolor{green!10} &  0.101$^{\phantom{\ddag}}$ \cellcolor{green!37} &  0.159 \cellcolor{red!33} &  0.172 \cellcolor{red!50} &  0.164 \cellcolor{red!39} &  0.157 \cellcolor{red!30} &  0.115 \cellcolor{green!19} &  0.114 \cellcolor{green!21} &  0.126 \cellcolor{green!6} & \textbf{0.091} \cellcolor{green!50} \\\cline{2-15}
& SemEval16 &  0.170 \cellcolor{green!31} &  0.306 \cellcolor{red!9} &  0.216 \cellcolor{green!17} &  0.148 \cellcolor{green!37} &  0.154$^{\phantom{\ddag}}$ \cellcolor{green!36} &  0.206 \cellcolor{green!20} &  0.183 \cellcolor{green!27} &  0.199 \cellcolor{green!22} &  0.248 \cellcolor{green!7} &  0.150 \cellcolor{green!37} &  0.150 \cellcolor{green!37} &  0.439 \cellcolor{red!50} & \textbf{0.108} \cellcolor{green!50} \\\cline{2-15}
& SST &  0.106 \cellcolor{red!10} &  0.126 \cellcolor{red!26} &  0.153 \cellcolor{red!50} &  0.051 \cellcolor{green!36} &  0.038$^{\dag\phantom{\dag}}$ \cellcolor{green!48} &  0.148 \cellcolor{red!45} &  0.110 \cellcolor{red!13} &  0.134 \cellcolor{red!33} &  0.131 \cellcolor{red!31} &  0.048 \cellcolor{green!40} & \textbf{0.036} \cellcolor{green!50} &  0.109 \cellcolor{red!12} &  0.053 \cellcolor{green!35} \\\cline{2-15}
& WA &  0.067 \cellcolor{red!4} &  0.056 \cellcolor{green!7} &  0.068 \cellcolor{red!5} &  0.025 \cellcolor{green!41} & \textbf{0.018}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.109 \cellcolor{red!50} &  0.092 \cellcolor{red!32} &  0.043 \cellcolor{green!22} &  0.054 \cellcolor{green!9} &  0.022 \cellcolor{green!45} &  0.022 \cellcolor{green!44} &  0.024 \cellcolor{green!42} &  0.034 \cellcolor{green!32} \\\cline{2-15}
& WB &  0.062 \cellcolor{red!6} &  0.030 \cellcolor{green!31} &  0.070 \cellcolor{red!15} &  0.019 \cellcolor{green!43} & \textbf{0.014}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.099 \cellcolor{red!50} &  0.069 \cellcolor{red!14} &  0.096 \cellcolor{red!46} &  0.052 \cellcolor{green!5} &  0.025 \cellcolor{green!37} &  0.021 \cellcolor{green!41} &  0.028 \cellcolor{green!33} &  0.026 \cellcolor{green!36} \\\cline{2-15}
\cline{2-15}
& Average &  0.109 \cellcolor{red!9} &  0.104$^{\ddag}$ \cellcolor{red!4} &  0.144 \cellcolor{red!49} &  0.066$^{\ddag}$ \cellcolor{green!39} & \textbf{0.056} \cellcolor{green!50} &  0.144 \cellcolor{red!50} &  0.134 \cellcolor{red!38} &  0.129 \cellcolor{red!32} &  0.143 \cellcolor{red!48} &  0.072$^{\ddag}$ \cellcolor{green!31} &  0.060$^{\ddag}$ \cellcolor{green!45} &  0.128$^{\ddag}$ \cellcolor{red!31} &  0.061$^{\ddag}$ \cellcolor{green!44} \\\hline

\multirow{12}{*}{\side{NKLD}} & GASP &  0.041 \cellcolor{green!5} &  0.022 \cellcolor{green!34} &  0.063 \cellcolor{red!29} &  0.014 \cellcolor{green!46} & \textbf{0.012}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.059 \cellcolor{red!23} &  0.056 \cellcolor{red!18} &  0.053 \cellcolor{red!13} &  0.076 \cellcolor{red!50} &  0.024 \cellcolor{green!31} &  0.015 \cellcolor{green!46} &  0.039 \cellcolor{green!7} &  0.014 \cellcolor{green!47} \\\cline{2-15}
& HCR &  0.070 \cellcolor{red!15} &  0.086 \cellcolor{red!39} &  0.093 \cellcolor{red!50} &  0.047 \cellcolor{green!20} &  0.031$^{\phantom{\ddag}}$ \cellcolor{green!43} &  0.085 \cellcolor{red!37} &  0.081 \cellcolor{red!32} &  0.076 \cellcolor{red!24} &  0.091 \cellcolor{red!46} &  0.038 \cellcolor{green!33} & \textbf{0.027} \cellcolor{green!50} &  0.039 \cellcolor{green!31} &  0.046 \cellcolor{green!21} \\\cline{2-15}
& OMD &  0.056 \cellcolor{red!0} &  0.049 \cellcolor{green!8} &  0.068 \cellcolor{red!18} &  0.038 \cellcolor{green!25} & \textbf{0.022}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.077 \cellcolor{red!32} &  0.065 \cellcolor{red!14} &  0.076 \cellcolor{red!30} &  0.059 \cellcolor{red!5} &  0.035 \cellcolor{green!29} &  0.030 \cellcolor{green!36} &  0.089 \cellcolor{red!50} &  0.039 \cellcolor{green!24} \\\cline{2-15}
& Sanders &  0.057 \cellcolor{red!9} &  0.024 \cellcolor{green!34} &  0.075 \cellcolor{red!33} &  0.015 \cellcolor{green!46} & \textbf{0.012}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.077 \cellcolor{red!36} &  0.077 \cellcolor{red!36} &  0.052 \cellcolor{red!3} &  0.087 \cellcolor{red!50} &  0.029 \cellcolor{green!27} &  0.020 \cellcolor{green!39} &  0.052 \cellcolor{red!3} &  0.031 \cellcolor{green!24} \\\cline{2-15}
& SemEval13 &  0.055 \cellcolor{red!0} &  0.043 \cellcolor{green!23} &  0.079 \cellcolor{red!50} &  0.038 \cellcolor{green!34} &  0.041$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.067 \cellcolor{red!24} &  0.078 \cellcolor{red!47} &  0.071 \cellcolor{red!33} &  0.078 \cellcolor{red!48} &  0.048 \cellcolor{green!13} &  0.040 \cellcolor{green!30} &  0.073 \cellcolor{red!38} & \textbf{0.030} \cellcolor{green!50} \\\cline{2-15}
& SemEval14 &  0.049 \cellcolor{red!2} &  0.028 \cellcolor{green!36} &  0.074 \cellcolor{red!50} &  0.025 \cellcolor{green!41} &  0.030$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.065 \cellcolor{red!34} &  0.065 \cellcolor{red!34} &  0.061 \cellcolor{red!26} &  0.071 \cellcolor{red!45} &  0.044 \cellcolor{green!5} &  0.027 \cellcolor{green!38} &  0.047 \cellcolor{green!1} & \textbf{0.021} \cellcolor{green!50} \\\cline{2-15}
& SemEval15 &  0.067 \cellcolor{red!4} &  0.057 \cellcolor{green!20} &  0.082 \cellcolor{red!42} &  0.061 \cellcolor{green!10} &  0.050$^{\phantom{\ddag}}$ \cellcolor{green!37} &  0.079 \cellcolor{red!33} &  0.085 \cellcolor{red!50} &  0.081 \cellcolor{red!39} &  0.078 \cellcolor{red!30} &  0.057 \cellcolor{green!19} &  0.057 \cellcolor{green!21} &  0.063 \cellcolor{green!6} & \textbf{0.045} \cellcolor{green!50} \\\cline{2-15}
& SemEval16 &  0.084 \cellcolor{green!28} &  0.140 \cellcolor{red!9} &  0.107 \cellcolor{green!13} &  0.073 \cellcolor{green!36} &  0.075$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.102 \cellcolor{green!16} &  0.090 \cellcolor{green!24} &  0.098 \cellcolor{green!19} &  0.122 \cellcolor{green!2} &  0.074 \cellcolor{green!35} &  0.074 \cellcolor{green!35} &  0.198 \cellcolor{red!50} & \textbf{0.054} \cellcolor{green!50} \\\cline{2-15}
& SST &  0.053 \cellcolor{red!10} &  0.062 \cellcolor{red!26} &  0.076 \cellcolor{red!50} &  0.026 \cellcolor{green!36} &  0.019$^{\dag\phantom{\dag}}$ \cellcolor{green!48} &  0.074 \cellcolor{red!45} &  0.055 \cellcolor{red!13} &  0.067 \cellcolor{red!34} &  0.065 \cellcolor{red!31} &  0.024 \cellcolor{green!40} & \textbf{0.018} \cellcolor{green!50} &  0.054 \cellcolor{red!12} &  0.027 \cellcolor{green!35} \\\cline{2-15}
& WA &  0.034 \cellcolor{red!4} &  0.028 \cellcolor{green!7} &  0.034 \cellcolor{red!5} &  0.013 \cellcolor{green!41} & \textbf{0.009}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.054 \cellcolor{red!50} &  0.046 \cellcolor{red!32} &  0.021 \cellcolor{green!22} &  0.027 \cellcolor{green!9} &  0.011 \cellcolor{green!45} &  0.011 \cellcolor{green!44} &  0.012 \cellcolor{green!42} &  0.017 \cellcolor{green!31} \\\cline{2-15}
& WB &  0.031 \cellcolor{red!6} &  0.015 \cellcolor{green!31} &  0.035 \cellcolor{red!15} &  0.010 \cellcolor{green!43} & \textbf{0.007}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.050 \cellcolor{red!50} &  0.035 \cellcolor{red!14} &  0.048 \cellcolor{red!46} &  0.026 \cellcolor{green!5} &  0.012 \cellcolor{green!37} &  0.010 \cellcolor{green!41} &  0.014 \cellcolor{green!33} &  0.013 \cellcolor{green!36} \\\cline{2-15}
\cline{2-15}
& Average &  0.054 \cellcolor{red!9} &  0.050$^{\ddag}$ \cellcolor{red!1} &  0.071 \cellcolor{red!49} &  0.033$^{\ddag}$ \cellcolor{green!39} & \textbf{0.028} \cellcolor{green!50} &  0.072 \cellcolor{red!50} &  0.067 \cellcolor{red!38} &  0.064 \cellcolor{red!32} &  0.071 \cellcolor{red!48} &  0.036$^{\ddag}$ \cellcolor{green!31} &  0.030$^{\ddag}$ \cellcolor{green!45} &  0.062$^{\dag\phantom{\dag}}$ \cellcolor{red!27} &  0.031$^{\ddag}$ \cellcolor{green!44} \\\hline

\multirow{12}{*}{\side{SE}} & GASP &  0.013 \cellcolor{green!10} &  0.005 \cellcolor{green!43} &  0.023 \cellcolor{red!28} &  0.003 \cellcolor{green!48} & \textbf{0.003}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.021 \cellcolor{red!19} &  0.020 \cellcolor{red!16} &  0.018 \cellcolor{red!9} &  0.028 \cellcolor{red!50} &  0.007 \cellcolor{green!35} &  0.004$^{\phantom{\ddag}}$ \cellcolor{green!47} &  0.012$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!48} \\\cline{2-15}
& HCR &  0.026 \cellcolor{red!8} &  0.017 \cellcolor{green!21} &  0.036 \cellcolor{red!44} &  0.009 \cellcolor{green!47} &  0.009$^{\phantom{\ddag}}$ \cellcolor{green!45} &  0.032 \cellcolor{red!31} &  0.031 \cellcolor{red!27} &  0.029 \cellcolor{red!19} &  0.038 \cellcolor{red!50} &  0.011 \cellcolor{green!41} & \textbf{0.008}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.008$^{\ddag}$ \cellcolor{green!49} &  0.015$^{\phantom{\ddag}}$ \cellcolor{green!26} \\\cline{2-15}
& OMD &  0.020 \cellcolor{red!10} &  0.013 \cellcolor{green!19} &  0.025 \cellcolor{red!34} &  0.008 \cellcolor{green!39} & \textbf{0.005}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.029 \cellcolor{red!50} &  0.024 \cellcolor{red!28} &  0.028 \cellcolor{red!46} &  0.022 \cellcolor{red!21} &  0.011 \cellcolor{green!27} &  0.009$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.023$^{\phantom{\ddag}}$ \cellcolor{red!26} &  0.013$^{\phantom{\ddag}}$ \cellcolor{green!15} \\\cline{2-15}
& Sanders &  0.020 \cellcolor{green!2} &  0.006 \cellcolor{green!43} &  0.029 \cellcolor{red!22} &  0.004 \cellcolor{green!47} & \textbf{0.003}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.029 \cellcolor{red!23} &  0.033 \cellcolor{red!32} &  0.018 \cellcolor{green!9} &  0.039 \cellcolor{red!50} &  0.009 \cellcolor{green!35} &  0.005$^{\phantom{\ddag}}$ \cellcolor{green!44} &  0.012$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.010$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-15}
& SemEval13 &  0.021 \cellcolor{green!2} &  0.012 \cellcolor{green!40} &  0.032 \cellcolor{red!45} & \textbf{0.010} \cellcolor{green!50} &  0.014$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.025 \cellcolor{red!14} &  0.033 \cellcolor{red!50} &  0.028 \cellcolor{red!26} &  0.033 \cellcolor{red!48} &  0.016 \cellcolor{green!21} &  0.014$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.020$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.010$^{\ddag}$ \cellcolor{green!49} \\\cline{2-15}
& SemEval14 &  0.017 \cellcolor{red!2} &  0.006 \cellcolor{green!45} &  0.028 \cellcolor{red!50} & \textbf{0.005} \cellcolor{green!50} &  0.009$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.024 \cellcolor{red!31} &  0.026 \cellcolor{red!39} &  0.023 \cellcolor{red!25} &  0.028 \cellcolor{red!47} &  0.014 \cellcolor{green!11} &  0.007$^{\phantom{\ddag}}$ \cellcolor{green!41} &  0.011$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.006$^{\phantom{\ddag}}$ \cellcolor{green!46} \\\cline{2-15}
& SemEval15 &  0.026 \cellcolor{red!2} &  0.018 \cellcolor{green!40} &  0.035 \cellcolor{red!49} & \textbf{0.016} \cellcolor{green!50} &  0.018$^{\phantom{\ddag}}$ \cellcolor{green!38} &  0.030 \cellcolor{red!25} &  0.035 \cellcolor{red!50} &  0.031 \cellcolor{red!32} &  0.033 \cellcolor{red!41} &  0.020 \cellcolor{green!28} &  0.019$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.017$^{\phantom{\ddag}}$ \cellcolor{green!42} &  0.016$^{\ddag}$ \cellcolor{green!48} \\\cline{2-15}
& SemEval16 &  0.032 \cellcolor{green!4} &  0.038 \cellcolor{red!12} &  0.043 \cellcolor{red!28} &  0.024 \cellcolor{green!29} &  0.019$^{\dag\phantom{\dag}}$ \cellcolor{green!46} &  0.041 \cellcolor{red!22} &  0.036 \cellcolor{red!8} &  0.040 \cellcolor{red!19} &  0.050 \cellcolor{red!50} &  0.028 \cellcolor{green!18} &  0.028$^{\phantom{\ddag}}$ \cellcolor{green!18} &  0.046$^{\phantom{\ddag}}$ \cellcolor{red!38} & \textbf{0.018}$^{\phantom{\ddag}}$ \cellcolor{green!50} \\\cline{2-15}
& SST &  0.018 \cellcolor{red!3} &  0.012 \cellcolor{green!22} &  0.030 \cellcolor{red!50} &  0.005 \cellcolor{green!47} & \textbf{0.005}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.027 \cellcolor{red!39} &  0.019 \cellcolor{red!6} &  0.024 \cellcolor{red!27} &  0.025 \cellcolor{red!32} &  0.006 \cellcolor{green!43} &  0.005$^{\ddag}$ \cellcolor{green!49} &  0.015$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.008$^{\phantom{\ddag}}$ \cellcolor{green!38} \\\cline{2-15}
& WA &  0.010 \cellcolor{green!3} &  0.005 \cellcolor{green!31} &  0.010 \cellcolor{green!3} &  0.003 \cellcolor{green!45} & \textbf{0.002}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.018 \cellcolor{red!50} &  0.015 \cellcolor{red!31} &  0.006 \cellcolor{green!26} &  0.008 \cellcolor{green!17} &  0.003 \cellcolor{green!45} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!47} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!45} &  0.005$^{\phantom{\ddag}}$ \cellcolor{green!36} \\\cline{2-15}
& WB &  0.009 \cellcolor{green!3} &  0.003 \cellcolor{green!41} &  0.011 \cellcolor{red!7} &  0.002 \cellcolor{green!48} & \textbf{0.002}$^{\phantom{\ddag}}$ \cellcolor{green!50} &  0.016 \cellcolor{red!43} &  0.011 \cellcolor{red!6} &  0.017 \cellcolor{red!50} &  0.007 \cellcolor{green!14} &  0.004 \cellcolor{green!37} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!43} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!40} &  0.003$^{\phantom{\ddag}}$ \cellcolor{green!39} \\\cline{2-15}
\cline{2-15}
& Average &  0.019 \cellcolor{red!4} &  0.012$^{\ddag}$ \cellcolor{green!30} &  0.027 \cellcolor{red!45} & \textbf{0.008} \cellcolor{green!50} &  0.008$^{\ddag}$ \cellcolor{green!49} &  0.027 \cellcolor{red!41} &  0.026 \cellcolor{red!37} &  0.024 \cellcolor{red!27} &  0.028 \cellcolor{red!50} &  0.012$^{\ddag}$ \cellcolor{green!32} &  0.009$^{\ddag}$ \cellcolor{green!43} &  0.016$^{\ddag}$ \cellcolor{green!12} &  0.010$^{\ddag}$ \cellcolor{green!41} \\\hline


                \end{tabular}%
                }
            

==> tab_results_mae.tex <==

        \begin{tabularx}{\textwidth}{|c||Y|Y|Y|Y|Y|Y|Y|Y||Y|} \hline
          & \multicolumn{8}{c||}{Methods tested in~\cite{Gao:2016uq}} &  \\ \hline
     & \side{CC$^{\mathrm{AE}}$}  & \side{ACC$^{\mathrm{AE}}$}  & \side{PCC$^{\mathrm{AE}}$}  & \side{PACC$^{\mathrm{AE}}$}  & \side{EMQ$^{\mathrm{AE}}$}  & \side{SVM(Q)$^{\mathrm{AE}}$}  & \side{SVM(KLD)$^{\mathrm{AE}}$}  & \side{SVM(NKLD)$^{\mathrm{AE}}$}  & \side{SVM(AE)$^{\mathrm{AE}}$} \\\hline
GASP & 0.103$\phantom{\dag}\phantom{\dag}$\cellcolor{red!16}& 0.057$\phantom{\dag}\phantom{\dag}$\cellcolor{green!29}& 0.137$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.059$\phantom{\dag}\phantom{\dag}$\cellcolor{green!27}& \textbf{0.036}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.119$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}& 0.114$\phantom{\dag}\phantom{\dag}$\cellcolor{red!27}& 0.109$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 0.136$\phantom{\dag}\phantom{\dag}$\cellcolor{red!49}\\\hline
HCR & 0.131$\phantom{\dag}\phantom{\dag}$\cellcolor{red!17}& 0.081$\phantom{\dag}\phantom{\dag}$\cellcolor{green!40}& 0.159$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.080$\phantom{\dag}\phantom{\dag}$\cellcolor{green!42}& \textbf{0.073}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.150$\phantom{\dag}\phantom{\dag}$\cellcolor{red!39}& 0.143$\phantom{\dag}\phantom{\dag}$\cellcolor{red!31}& 0.138$\phantom{\dag}\phantom{\dag}$\cellcolor{red!24}& 0.157$\phantom{\dag}\phantom{\dag}$\cellcolor{red!47}\\\hline
OMD & 0.122$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 0.079$\phantom{\dag}\phantom{\dag}$\cellcolor{green!38}& 0.129$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}& 0.081$\phantom{\dag}\phantom{\dag}$\cellcolor{green!36}& \textbf{0.071}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.141$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.124$\phantom{\dag}\phantom{\dag}$\cellcolor{red!26}& 0.139$\phantom{\dag}\phantom{\dag}$\cellcolor{red!46}& 0.116$\phantom{\dag}\phantom{\dag}$\cellcolor{red!14}\\\hline
Sanders & 0.128$\phantom{\dag}\phantom{\dag}$\cellcolor{red!24}& 0.062$\phantom{\dag}\phantom{\dag}$\cellcolor{green!35}& 0.149$\phantom{\dag}\phantom{\dag}$\cellcolor{red!42}& 0.062$\phantom{\dag}\phantom{\dag}$\cellcolor{green!34}& \textbf{0.046}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.140$\phantom{\dag}\phantom{\dag}$\cellcolor{red!34}& 0.140$\phantom{\dag}\phantom{\dag}$\cellcolor{red!35}& 0.110$\phantom{\dag}\phantom{\dag}$\cellcolor{red!7}& 0.157$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}\\\hline
SemEval13 & 0.117$\phantom{\dag}\phantom{\dag}$\cellcolor{red!9}& 0.089$\phantom{\dag}\phantom{\dag}$\cellcolor{green!34}& 0.144$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& \textbf{0.078}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.093$\phantom{\dag}\phantom{\dag}$\cellcolor{green!28}& 0.129$\phantom{\dag}\phantom{\dag}$\cellcolor{red!27}& 0.144$\phantom{\dag}\phantom{\dag}$\cellcolor{red!49}& 0.134$\phantom{\dag}\phantom{\dag}$\cellcolor{red!35}& 0.143$\phantom{\dag}\phantom{\dag}$\cellcolor{red!49}\\\hline
SemEval14 & 0.106$\phantom{\dag}\phantom{\dag}$\cellcolor{red!8}& 0.071$\phantom{\dag}\phantom{\dag}$\cellcolor{green!40}& 0.136$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& \textbf{0.064}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.073$\phantom{\dag}\phantom{\dag}$\cellcolor{green!37}& 0.127$\phantom{\dag}\phantom{\dag}$\cellcolor{red!37}& 0.128$\phantom{\dag}\phantom{\dag}$\cellcolor{red!38}& 0.122$\phantom{\dag}\phantom{\dag}$\cellcolor{red!30}& 0.134$\phantom{\dag}\phantom{\dag}$\cellcolor{red!47}\\\hline
SemEval15 & 0.129$\phantom{\dag}\phantom{\dag}$\cellcolor{red!9}& 0.108$\phantom{\dag}\phantom{\dag}$\cellcolor{green!30}& 0.149$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.112$\phantom{\dag}\phantom{\dag}$\cellcolor{green!22}& \textbf{0.098}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.142$\phantom{\dag}\phantom{\dag}$\cellcolor{red!36}& 0.149$\phantom{\dag}\phantom{\dag}$\cellcolor{red!49}& 0.144$\phantom{\dag}\phantom{\dag}$\cellcolor{red!39}& 0.144$\phantom{\dag}\phantom{\dag}$\cellcolor{red!38}\\\hline
SemEval16 & 0.148$\phantom{\dag}\phantom{\dag}$\cellcolor{red!11}& 0.157$\phantom{\dag}\phantom{\dag}$\cellcolor{red!23}& 0.176$\phantom{\dag}\phantom{\dag}$\cellcolor{red!47}& 0.125$\phantom{\dag}\phantom{\dag}$\cellcolor{green!17}& \textbf{0.100}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.167$\phantom{\dag}\phantom{\dag}$\cellcolor{red!35}& 0.154$\phantom{\dag}\phantom{\dag}$\cellcolor{red!19}& 0.164$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}& 0.178$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}\\\hline
SST & 0.115$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 0.082$\phantom{\dag}\phantom{\dag}$\cellcolor{green!15}& 0.138$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.079$\phantom{\dag}\phantom{\dag}$\cellcolor{green!18}& \textbf{0.052}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.136$\phantom{\dag}\phantom{\dag}$\cellcolor{red!47}& 0.113$\phantom{\dag}\phantom{\dag}$\cellcolor{red!20}& 0.128$\phantom{\dag}\phantom{\dag}$\cellcolor{red!38}& 0.125$\phantom{\dag}\phantom{\dag}$\cellcolor{red!34}\\\hline
WA & 0.081$\phantom{\dag}\phantom{\dag}$\cellcolor{red!5}& 0.046$\phantom{\dag}\phantom{\dag}$\cellcolor{green!44}& 0.083$\phantom{\dag}\phantom{\dag}$\cellcolor{red!8}& \textbf{0.043}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.043$\dag\dag$\cellcolor{green!49}& 0.111$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.100$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}& 0.063$\phantom{\dag}\phantom{\dag}$\cellcolor{green!19}& 0.071$\phantom{\dag}\phantom{\dag}$\cellcolor{green!8}\\\hline
WB & 0.081$\phantom{\dag}\phantom{\dag}$\cellcolor{red!15}& 0.044$\phantom{\dag}\phantom{\dag}$\cellcolor{green!36}& 0.084$\phantom{\dag}\phantom{\dag}$\cellcolor{red!19}& 0.041$\phantom{\dag}\phantom{\dag}$\cellcolor{green!39}& \textbf{0.034}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 0.106$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 0.084$\phantom{\dag}\phantom{\dag}$\cellcolor{red!19}& 0.103$\phantom{\dag}\phantom{\dag}$\cellcolor{red!46}& 0.069$\phantom{\dag}\phantom{\dag}$\cellcolor{green!0}\\\hline
\end{tabularx}

    

==> tab_results_mrae.tex <==
\begin{tabularx}{\textwidth}{|c||Y|Y|Y|Y|Y|Y|Y|Y||Y|} \hline
          & \multicolumn{8}{c||}{Methods tested in~\cite{Gao:2016uq}} &  \\ \hline
     & \side{CC$^{\mathrm{RAE}}$}  & \side{ACC$^{\mathrm{RAE}}$}  & \side{PCC$^{\mathrm{RAE}}$}  & \side{PACC$^{\mathrm{RAE}}$}  & \side{EMQ$^{\mathrm{RAE}}$}  & \side{SVM(Q)$^{\mathrm{RAE}}$}  & \side{SVM(KLD)$^{\mathrm{RAE}}$}  & \side{SVM(NKLD)$^{\mathrm{RAE}}$}  & \side{SVM(RAE)$^{\mathrm{RAE}}$} \\\hline
GASP & 2.974$\phantom{\dag}\phantom{\dag}$\cellcolor{red!11}& 0.690$\phantom{\dag}\phantom{\dag}$\cellcolor{green!43}& 3.707$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}& 0.683$\phantom{\dag}\phantom{\dag}$\cellcolor{green!43}& \textbf{0.426}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.076$\phantom{\dag}\phantom{\dag}$\cellcolor{red!37}& 3.261$\phantom{\dag}\phantom{\dag}$\cellcolor{red!18}& 3.433$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 4.581$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}\\\hline
HCR & 3.866$\phantom{\dag}\phantom{\dag}$\cellcolor{red!25}& 1.344$\phantom{\dag}\phantom{\dag}$\cellcolor{green!31}& 4.292$\phantom{\dag}\phantom{\dag}$\cellcolor{red!35}& 1.517$\phantom{\dag}\phantom{\dag}$\cellcolor{green!27}& \textbf{0.512}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.934$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 4.219$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}& 4.187$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}& 3.998$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}\\\hline
OMD & 3.701$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}& 0.891$\phantom{\dag}\phantom{\dag}$\cellcolor{green!41}& 3.856$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}& 1.106$\phantom{\dag}\phantom{\dag}$\cellcolor{green!35}& \textbf{0.531}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.571$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 3.865$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}& 4.486$\phantom{\dag}\phantom{\dag}$\cellcolor{red!47}& 3.295$\phantom{\dag}\phantom{\dag}$\cellcolor{red!18}\\\hline
Sanders & 3.255$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 1.042$\phantom{\dag}\phantom{\dag}$\cellcolor{green!30}& 3.772$\phantom{\dag}\phantom{\dag}$\cellcolor{red!34}& 1.076$\phantom{\dag}\phantom{\dag}$\cellcolor{green!30}& \textbf{0.249}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.408$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 3.596$\phantom{\dag}\phantom{\dag}$\cellcolor{red!30}& 3.550$\phantom{\dag}\phantom{\dag}$\cellcolor{red!29}& 3.741$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}\\\hline
SemEval13 & 3.169$\phantom{\dag}\phantom{\dag}$\cellcolor{red!26}& 1.209$\phantom{\dag}\phantom{\dag}$\cellcolor{green!28}& 3.730$\phantom{\dag}\phantom{\dag}$\cellcolor{red!42}& 1.111$\phantom{\dag}\phantom{\dag}$\cellcolor{green!31}& \textbf{0.465}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.007$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 3.726$\phantom{\dag}\phantom{\dag}$\cellcolor{red!42}& 3.945$\phantom{\dag}\phantom{\dag}$\cellcolor{red!48}& 3.557$\phantom{\dag}\phantom{\dag}$\cellcolor{red!37}\\\hline
SemEval14 & 3.149$\phantom{\dag}\phantom{\dag}$\cellcolor{red!26}& 0.892$\phantom{\dag}\phantom{\dag}$\cellcolor{green!35}& 3.728$\phantom{\dag}\phantom{\dag}$\cellcolor{red!41}& 0.928$\phantom{\dag}\phantom{\dag}$\cellcolor{green!34}& \textbf{0.343}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.033$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 3.545$\phantom{\dag}\phantom{\dag}$\cellcolor{red!36}& 3.754$\phantom{\dag}\phantom{\dag}$\cellcolor{red!42}& 3.377$\phantom{\dag}\phantom{\dag}$\cellcolor{red!32}\\\hline
SemEval15 & 3.638$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}& 2.054$\phantom{\dag}\phantom{\dag}$\cellcolor{green!16}& 4.079$\phantom{\dag}\phantom{\dag}$\cellcolor{red!40}& 2.128$\phantom{\dag}\phantom{\dag}$\cellcolor{green!14}& \textbf{0.844}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.414$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 4.032$\phantom{\dag}\phantom{\dag}$\cellcolor{red!39}& 4.274$\phantom{\dag}\phantom{\dag}$\cellcolor{red!46}& 3.841$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}\\\hline
SemEval16 & 4.641$\phantom{\dag}\phantom{\dag}$\cellcolor{red!31}& 2.676$\phantom{\dag}\phantom{\dag}$\cellcolor{green!15}& 5.244$\phantom{\dag}\phantom{\dag}$\cellcolor{red!45}& 2.650$\phantom{\dag}\phantom{\dag}$\cellcolor{green!16}& \textbf{1.222}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 5.433$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 4.887$\phantom{\dag}\phantom{\dag}$\cellcolor{red!37}& 5.263$\phantom{\dag}\phantom{\dag}$\cellcolor{red!45}& 4.990$\phantom{\dag}\phantom{\dag}$\cellcolor{red!39}\\\hline
SST & 4.117$\phantom{\dag}\phantom{\dag}$\cellcolor{red!41}& 0.996$\phantom{\dag}\phantom{\dag}$\cellcolor{green!37}& 4.234$\phantom{\dag}\phantom{\dag}$\cellcolor{red!44}& 0.983$\phantom{\dag}\phantom{\dag}$\cellcolor{green!37}& \textbf{0.512}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 4.437$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 3.608$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}& 3.563$\phantom{\dag}\phantom{\dag}$\cellcolor{red!27}& 3.772$\phantom{\dag}\phantom{\dag}$\cellcolor{red!33}\\\hline
WA & 2.549$\phantom{\dag}\phantom{\dag}$\cellcolor{red!20}& 0.753$\phantom{\dag}\phantom{\dag}$\cellcolor{green!35}& 2.645$\phantom{\dag}\phantom{\dag}$\cellcolor{red!23}& 0.827$\phantom{\dag}\phantom{\dag}$\cellcolor{green!32}& \textbf{0.273}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 3.520$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 2.830$\phantom{\dag}\phantom{\dag}$\cellcolor{red!28}& 1.413$\phantom{\dag}\phantom{\dag}$\cellcolor{green!14}& 1.745$\phantom{\dag}\phantom{\dag}$\cellcolor{green!4}\\\hline
WB & 2.458$\phantom{\dag}\phantom{\dag}$\cellcolor{red!18}& 0.548$\phantom{\dag}\phantom{\dag}$\cellcolor{green!41}& 2.587$\phantom{\dag}\phantom{\dag}$\cellcolor{red!22}& 0.615$\phantom{\dag}\phantom{\dag}$\cellcolor{green!39}& \textbf{0.266}$\phantom{\dag}\phantom{\dag}$\cellcolor{green!50}& 3.456$\phantom{\dag}\phantom{\dag}$\cellcolor{red!50}& 2.534$\phantom{\dag}\phantom{\dag}$\cellcolor{red!21}& 2.255$\phantom{\dag}\phantom{\dag}$\cellcolor{red!12}& 1.954$\phantom{\dag}\phantom{\dag}$\cellcolor{red!2}\\\hline
\end{tabularx}

